LEGO-RL: Harness-Native Reinforcement Learning for Coding Agents

Reinforcement learning for coding agents increasingly relies on long-running agent harnesses to manage tool integration, repository contexts, and execution feedback. However, the native execution environments of these harnesses are inherently misaligned with policy-gradient training: environmental crashes and reward hacking corrupt outcome signals, while train-inference discrepancies decouple rollout behavior from policy updates. To address this, we present LEGO-RL, a framework that bridges native coding-agent harnesses with scalable policy-gradient optimization without modifying their internal control flow. LEGO-RL is built upon three pillars: (1) faithful optimization via in-process LLM proxying that captures raw generation streams for token-level alignment and robust trainer-side log-probability recomputation, even under harness-side compaction or re-serialization; (2) reliable execution via scalable sandbox orchestration featuring image caching and stage-wise defenses to mitigate reward hacking; and (3) observable training through an integrated plugin that automates validation and monitoring, paired with a Live UI for granular trajectory diagnostics. We evaluate LEGO-RL by training the sparse MoE model Qwen3.5-35B-A3B with GSPO across three native coding-agent harnesses. LEGO-RL improves Qwen3.5-35B-A3B across OpenHands SDK (64.0% to 70.4%), Claude Code (62.4% to 68.2%), and OpenCode (57.2% to 66.6%) on SWE-bench Verified, while maintaining a rollout-training probability correlation above 0.99.

==> tab_nydus.tex <==
% Nydus vs OCI sandbox-image delivery -- infrastructure A/B.
% Generated from the 2026-07-27 run on the 243 CPU sandbox cluster.
% \input{tab_nydus} ; needs booktabs.
% \begin{table}[t]
%     \centering
%     \small
%     \setlength{\tabcolsep}{6pt}
%     \begin{tabular}{lcccc c}
%         \toprule
%         & \multicolumn{2}{c}{Nydus} & \multicolumn{2}{c}{OCI} & \\
%         \cmidrule(lr){2-3} \cmidrule(lr){4-5}
%         Median per start & cold & warm & cold & warm & Ratio\textsuperscript{\dag} \\
%         \midrule
%         Pull (s)          & 0.10 & ---  & 1.29  & ---  & 12.8$\times$ \\
%         Ready (s)         & 1.57 & 0.64 & 2.66  & 0.78 & 1.7$\times$ \\
%         \quad max (s)     & 1.73 & ---  & 39.69 & ---  & 23$\times$ \\
%         Network (MB)      & 16.8 & 0.1  & 94.7  & 0.1  & 5.6$\times$ \\
%         Disk (MB)         & 56.2 & 0.1  & 238.0 & 0.1  & 4.2$\times$ \\
%         Read (MB/s)       & 63   & 105  & 339   & 362  & 0.19$\times$ \\
%         \bottomrule
%     \end{tabular}
%     \caption{\textbf{Nydus lazy pull vs.\ conventional OCI pull for sandbox
%     images.} The same 100 SWE-bench Verified instances are measured in all four
%     cells ($n{=}100$ each, paired by instance and node); \emph{cold} means the
%     image was verifiably absent from that node beforehand, \emph{warm} is an
%     immediate re-run of the identical pod. The win is in the tail, not the
%     median. Aggregated over 100 starts: $1.59$ vs.\ $21.6$\,GB over the wire and
%     $5.29$ vs.\ $65.6$\,GB written to disk.
%     \textsuperscript{\dag}OCI\,$\div$\,Nydus, cold column; for read throughput
%     $<1$ means Nydus is slower. Entry point is a probe script, so these are
%     infrastructure numbers---no LLM, no agent loop, no reward.}
%     \label{tab:nydus}
% \end{table}

